Elementary Real Analysis

Preliminary version of a book on univariate real analysis, with 19 chapters and 6 appendices. 1. Prologue on functions and relations; 2. From ZFC formulas to natural numbers; 3. From natural numbers to integers; 4. From integers to fractions; 5. From fractions to extended reals; 6. From extended reals to real numbers; 7. Limits of real sequences; 8. Infinite series; 9. Limits of real functions. 10. Elementary functions; 11. Continuous functions; 12. Derivatives; 13. Mean value theorems; 14. Taylor polynomials; 15. Real analytic functions; 16. Newton integral; 17. Riemann integral; 18. Henstock-Kurzweil integral; 19. Applications of integrals; A. ZFC set theory; B. The equiconsistence of AC: G\"odel; C. The equiconsistence of $\neg$AC: Cohen; D. From real numbers to complex numbers; E. Metric spaces; F. Solutions to exercises

==> lec10.tex <==
\chapter[Primitives of uniformly continuous functions]{Primitives of UC functions}\label{chap_pr10}

The 10th chapter is based on lecture~10 
\begin{quote}
\url{https://kam.mff.cuni.cz/~klazar/MAI24_pred10.pdf}    
\end{quote}
given on April 25, 2024, but we transformed the lecture considerably. 
We generalize the classical result that every continuous function 
$$
f\cc[a,\,b]\to\R\,,
$$ 
which by Theorem~\ref{thm_steSpo} is even uniformly continuous, has 
a~primitive function and prove the following.

\begin{thm}[primitives of UC functions]\label{thm_primUC}
Let $M\sus\R$ be bounded and $f\cc M\to\R$ be uniformly 
continuous. \underline{Then} there is a~function $F\in\mathcal{F}(M)$ such 
that    
$$
F'(b)=f(b)
$$
for every point $b\in M$ that is not isolated.
\end{thm}
Section~\ref{sec_twoKRint} is devoted to the proof of this theorem.

In Section~\ref{sec_antider} we review basic properties of primitive functions. 
In Definition~\ref{def_globPrim} we invert the operation of global 
derivative. Theorem~\ref{thm_primOnInter} is the classical result that every two primitives 
of a~function defined on an interval differ by a~constant. In the proof of 
Theorem~\ref{thm_gluePrim} we show how to glue infinitely many primitives on intervals.

\section{Global antiderivative}\label{sec_antider}

We investigate inversion of the operation 
$f\mapsto f'$ of global derivative on $\mathcal{R}$.

\medskip\noindent
{\em $\bullet$ Global primitive. }Let $F,f\in\mathcal{R}$. The function $F$ is an \underline{antiderivative\index{antiderivative|emph}}, or 
a~\underline{primitive\index{primitive|emph}}, of the function $f$ if $M(F)=M(f)$ and $F'=f$. Then we write 
$${\textstyle
F=\int f\,.\label{integral}
}
$$

\begin{exer}\label{ex_priklNaPrim}
Find functions $F,f\in\mathcal{R}$ such that $F'=f$ but 
$F\ne\int f$.
\end{exer}

\begin{exer}\label{ex_primCont}
If $F=\int f$ then $F\in\mathcal{C}$.    
\end{exer}
After addition, multiplication, division, composition, inverse 
(Definition~\ref{def_oprOnR}) and global
derivative (Definition~\ref{def_deriFunk}) we 
introduce a~seventh operation on $\mathcal{R}$, the global primitive. It
is an ``inverse'' of the global derivative.
Recall that for any set $X$ we denote by $\mathcal{P}(X)$ the power set of $X$, 
the set of all subsets of $X$.

\begin{defi}[global primitive]\label{def_globPrim}
The map
$$
{\textstyle
\int\cc\mathcal{R}\to\mathcal{P}(\mathcal{R}),\ \int(f)\equiv\{F\in\mathcal{R}\cc\;F=\int f\}\,,
}
$$
is the \underline{global primitive\index{global primitive|emph}}.\label{globPrimi}
\end{defi}
Unlike the previous six operations, $\int$ is not really an operation 
on $\mathcal{R}$, it is a~multioperation on $\mathcal{R}$. 
It associates to every $f\in\mathcal{R}$  not one value in $\mathcal{R}$, but 
a~set of values.  

\begin{exer}\label{ex_prim1}
If $F=\int f$ then $F+c=\int f$ for every $c\in\R$.     
\end{exer}

Recall that $\emptyset_f=\langle
\emptyset,\R,\emptyset\rangle$ ($\in\mathcal{R}$) is the empty real 
function. 

\begin{prop}[a~trichotomy]\label{prop_atricho}
Let $g\in\mathcal{R}$. \underline{Then} the following three cases occur for the set $\int(g)$.
\begin{enumerate}
\item If $g=\emptyset_f$ then
$\int(g)=\{\emptyset_f\}$.
\item $\int(g)=\emptyset$.
\item The set $\int(g)$ is uncountable.
\end{enumerate}
\end{prop}
\duk
Part~1 holds trivially. Suppose that $g\ne\emptyset_f$, $G\in\int(g)$ and 
$b\in M(g)$. By the previous exercise, $G+c\in\int(g)$ for every $c$. We have 
$$
c\ne c'\Rightarrow G+c\ne G+c'
$$ because 
$(G+c)(b)\ne (G+c')(b)$ (this fails for $G=\emptyset_f$). Thus the map
$$
c\mapsto G+c
$$
is an injection from $\R$ to $\int(g)$ and the last set is uncountable. This proves that for $g\ne\emptyset_f$ either case~2 or case~3 occurs.
\kduk

\noindent
It is not known for which $f$ case~2 occurs. Thus $\int$ is the most complex 
of the seven operations on $\mathcal{R}$. 

If $M(f)\not\sus L(M(f))$, for example if $M(f)=\{b\}$, then
$\int(f)=\emptyset$. More positively,
$\mathrm{e}^x=\int \mathrm{e}^x$ and we show soon that
$$
{\textstyle
\int\big(\mathrm{e}^x\big)=\{\mathrm{e}^x+c\cc\;c\in\R\}\,.
}
$$

\noindent
{\em $\bullet$ Primitives on nontrivial intervals. }We investigate properties of
antiderivatives of functions defined on nontrivial intervals.

\begin{thm}[primitives on intervals]\label{thm_primOnInter}
Suppose\index{theorem!primitives on intervals|emph} that $I$ is a~nontrivial interval and functions $F$, $G$ and $f$ in $\mathcal{F}(I)$ are such that 
$${\textstyle
F=\int f\,\text{ and }\,G=\int f\,.
}
$$
\underline{Then} there is a~number $c\in\R$ such that
$$
F(x)=G(x)+k_c(x)\,.
$$
\end{thm}
\duk
Let $a<b$ be in $I$. By 
Theorem~\ref{thm_Lagrange} for the interval $[a,b]$ and function $(F-G)\,|\,[a,b]$ there is a~number $c\in(a,b)$ 
such that
\begin{eqnarray*}
(F(b)-G(b))-(F(a)-G(a))&=&(F(x)-G(x))'(c)\cdot(b-a)\\
&=&(f(c)-f(c))\cdot(b-a)=0\,.
\end{eqnarray*}
Thus 
$$
F(b)-G(b)=F(a)-G(a)\,.
$$
It follows that $F-G=k_c\,|\,I$ for some $c\in\R$, hence $F=G+k_c$.
\kduk

\begin{cor}[primitives on intervals]\label{cor_primOnInter}
Suppose that $I$ is a~nontrivial interval and $f\in\mathcal{F}(I)$ is a~function such 
that $\int(f)\ne\emptyset$. \underline{Then} there exists a~function
$F\in\mathcal{F}(I)$ such that
$${\textstyle
\int(f)=\{F+c\cc\;c\in\R\}\,.
}
$$
\end{cor}
\duk
Let $F\in\int(f)$ be arbitrary. It is clear then that $F+c\in\int(f)$ for every $c\in\R$. On the other hand, if $G\in\int(f)$, then $G=F+c$ by Theorem~\ref{thm_primOnInter}.
\kduk
\vspace{-3mm}
\begin{exer}\label{ex_FvteRoli}
Every such function $F$ is in $\int(f)$ and every function in $\int(f)$ can play 
the role of the function $F$.
\end{exer}
Thus if $M(g)$ is a~nontrivial interval, we can make case~3 of Proposition~\ref{prop_atricho} more precise: the set $\int(g)$ is in bijection with $\R$.

\begin{thm}[gluing primitives]\label{thm_gluePrim}
Let\index{theorem!gluing primitives|emph}
$$
I_1\sus I_2\sus\ds
$$
be nested nontrivial intervals, $I\equiv\bigcup_{n=1}^{\infty}$ and 
$f\in\mathcal{F}(I)$ be such function that $\int(f\,|\,I_n)\ne\emptyset$ for 
every $n$. \underline{Then} $I$ is a~nontrivial interval and 
$${\textstyle
\int(f)\ne\emptyset\,.
}
$$
\end{thm}
\duk
Since $I\supset I_1$, we have $I\ne\emptyset,\{b\}$. If $a<b<c$ with 
$a,c\in I$, then there is an $n$ such that $a,c\in I_n$ (Exercise~\ref{ex_procInter}). Since 
$I_n$ is an interval, $b\in I_n$ and $b\in I$. Thus $I$ is a~nontrivial 
interval.

We take an arbitrary $F_1\in\int(f\,|\,I_1)$. Suppose that 
$n\in\N$ and that functions $F_i\in\int(f\,|\,I_i)$ for $i\in[n]$ are selected such that ($F_0\equiv{\emptyset_f}$)
$$
\text{$G_{F_{i-1}}\sus G_{F_i}$ for $i\in[n]$}\,.
$$
To get $F_{n+1}$, we take any $F\in\int(f\,|\,I_{n+1})$. Then $F\,|\,I_n\in\int(f\,|\,I_n)$ and by Theorem~\ref{thm_primOnInter} there is a~number $c\in\R$ such that
$$
F\,|\,I_n=F_n+k_c\,.
$$
We set $F_{n+1}\equiv F-k_c$. Then 
$F_{n+1}\in\int(f\,|\,I_{n+1})$ and 
$$
\text{$F_{n+1}\,|\,I_n=F_n$, that is, 
$G_{F_n}\sus G_{F_{n+1}}$}\,.
$$
Finally, we define the desired primitive function $F$ of $f$ via its graph:
$${\textstyle
G_F\equiv\bigcup_{n=1}^{\infty}G_{F_n}\,.
}
$$
We check that $F=\int f$. Let $a\in I$ be arbitrary. There is an index $n$ such that $a\in I_n$. Moreover, $n$ can be selected so that if $a\in I^0$ then also $a\in I_n^0$ (Exercise~\ref{ex_explInterv}). We take such index $n$ and, since $F\,|\,I_n=F_n$, we have (due to the locality of derivative) that
$$
F'(a)=\big(F\,|\,I_n\big)'(a)=F_n'(a)=
f(a)\,,
$$
as required. 
\kduk
\vspace{-3mm}
\begin{exer}\label{ex_procInter}
Why does such an $n$ exist?    
\end{exer}

\begin{exer}\label{ex_explInterv}
Explain why such index $n$ exists and why we need it, that is, why it does not 
suffice that $a\in I_n$.     
\end{exer}

\begin{exer}\label{ex_PrimEvInt}
Show that if every function $f\in\mathcal{C}([a,b])$, $a<b$, has an 
antiderivative, then every function $f\in\mathcal{C}(I)$, where $I$ is 
a~nontrivial interval, has an antiderivative.
\end{exer}

\noindent
{\em $\bullet$ Global primitive and addition. }For two sets $A,B\sus\mathcal{R}$ we set
$$
A+B\equiv\{f+g\cc\;f\in A,\,g\in B\}\,.
$$
If $A=\emptyset$ or $B=\emptyset$, then $A+B=\emptyset$.

\begin{thm}[$\int+\int \sus\int$]\label{thm_GlPriAdd}
Let\index{theorem!primitives of sums|emph} 
$f,g\in\mathcal{R}$ be such that $\int(f+g)\ne\emptyset$. \underline{Then}
$${\textstyle
\int(f)+\int(g)\sus\int(f+g)\,.
}
$$
\end{thm}
\duk
If $\int(f+g)=\{\emptyset_f\}$ or 
$\int(f)=\emptyset$ or $\int(g)=\emptyset$, the inclusion trivially holds. We assume that $\int(f+g)\ne \emptyset, 
\{\emptyset_f\}$, and that $F\in\int f$ 
and $G\in\int g$. Then
$$
M\equiv M(F+G)=M(f+g)=M(f)\cap M(g)
$$
and $M\sus L(M)$.
For every $a\in M$ we have by part~1 of Theorem~\ref{thm_nasob} that
$$
(F+G)'(a)=F'(a)+G'(a)=f(a)+g(a)=(f+g)(a)\,.
$$
Thus $F+G\in\int(f+g)$.
\kduk

\noindent
The inclusion $\int(f)+\int(g)\sus\int(f+g)$ may be strict. For example, for $f\equiv\sgn\,x$ and
$g\equiv-\sgn\,x$ we have
$$
{\textstyle
\int(f)=\int(g)=\emptyset\,\text{ and }\,
\int(f+g)=\{k_c(x)\cc\;c\in\R\}\,.
}
$$
Emptiness of the first two sets follows from Corollary~\ref{cor_Darbouxe} 
below. The structure of the last set follows from
Corollary~\ref{cor_primOnInter}. The assumption $\int(f+g)\ne\emptyset$ is 
necessary. For example, if $f\equiv k_0\,|\,[-1,0]$ and $g\equiv 
k_0\,|\,[0,1]$, then
$$
{\textstyle
\int(f)+\int(g)=\{k_c\,|\,\{0\}\cc\;c\in\R\}\,\text{ but }\,\int(f+g)=\emptyset\,.
}
$$

We describe a~situation where we have equality $\int(f)+\int(g)=\int(f+g)$.

\begin{prop}[$\int+\int=\int$]\label{prop_sumIntEqu}
Suppose that $f,g\in\mathcal{R}$, $M(f)$ and $M(g)$ are intervals and that 
$${\textstyle
\int(f),\,\int(g),\, \int(f+g)\ne\emptyset,\,\{\emptyset_f\}\,.
}
$$
\underline{Then}
$${\textstyle
\int(f)+\int(g)=\int(f+g)\,.
}
$$
\end{prop}
\duk
Let $F\in\int(f)$ and $G\in\int(g)$. Since $M(f+g)$ is a~nontrivial 
interval, we have $F+G\in\int(f+g)$. By Corollary~\ref{cor_primOnInter} and Exercise~\ref{ex_FvteRoli},
\begin{eqnarray*}
{\textstyle
\int(f)+\int(g)}&=&\{F+k_c\cc\;c\in\R\}+
\{G+k_d\cc\;c\in\R\}\\
&=&\{F+G+k_c+k_d\cc\;c,\,d\in\R\}\\
&=&\{F+G+k_c\cc\;c\in\R\}={\textstyle
\int(f+g)}\,.
\end{eqnarray*}
\kduk
\vspace{-3mm}
\begin{exer}\label{ex_adapDiff}
Adapt Theorem~\ref{thm_GlPriAdd} and Proposition~\ref{prop_sumIntEqu} for the difference $\int(f)-\int(g)$.    
\end{exer}

For the reader's convenience we give, as an exercise, the standard formula for the primitive of a~sum, resp. difference. 

\begin{exer}\label{ex_explDifNot}
Prove the next proposition.
\end{exer}

\begin{prop}[standard $\int(f\pm g)$]\label{prop_standPriSum}
If $f,g,F,G\in\mathcal{F}(I)$ are such that $F=\int f$, $G=\int g$ and $I$ is 
a~nontrivial interval, \underline{then}, with equals signs,  
$$
{\textstyle
F\pm g=\int(f\pm g)\,.
}
$$  
\end{prop}

\noindent
{\em $\bullet$ A~theorem on primitives due to J.-G.~Darboux. }{\em Jean-Gaston 
Darboux (1842--1917)\index{Darboux, Jean-Gaston}} was a~French mathematician. We will meet him again in 
connection with definitions
of Riemann integral. 

\begin{thm}[Darboux's 1]\label{thm_deriDarboux}
Let\index{theorem!Darboux's|emph} 
$I$ be a~nontrivial interval, $f\in\mathcal{F}(I)$ and 
$\int(f)\ne\emptyset$. If $a<b$ in $I$ and $c$ are real numbers such that
$$
f(a)<c<f(b)\vee f(a)>c>f(b)\,,
$$
\underline{then} there is a~number $d\in(a,b)$ such that
$$
f(d)=c\,.
$$
\end{thm}
\duk
Let $I$, $f$, $a$, $b$ and $c$ be as stated. We deal only with the case
$$
f(a)<c<f(b)\,,
$$
the case $f(a)>c>f(b)$ is treated similarly (Exercise~\ref{ex_how}). We take any $F\in\int(f)$ and consider the function
$$
G(x)\equiv F(x)-cx\,.
$$
By Exercise~\ref{ex_primCont} we have $G\in\mathcal{C}([a,b])$. By 
Corollary~\ref{cor_priMaxi} the function $G$ attains at some point $d\in[a,b]$ 
global minimum. From
$$
G'(a)=F'(a)-c=f(a)-c<0\,\text{ and, similarly, }\,G'(b)>0\,,
$$
and from Proposition~\ref{prop_deriMono2} we get that $d\in(a,b)$. From Theorem~\ref{thm_priznakExtr} we get that
$$
0=G'(d)=F'(d)-c=f(d)-c\,,
$$
and $f(d)=c$.
\kduk
\vspace{-3mm}
\begin{exer}\label{ex_how}
Modify the proof for the case $f(a)<c<f(b)$
\end{exer}

\begin{cor}[Darboux's 2]\label{cor_Darb}
Let $I$ be a~nontrivial interval, $f\in\mathcal{F}(I)$ and 
$\int(f)\ne\emptyset$. \underline{Then} for every interval $J\sus I$,
$$
\text{the image $f[J]$ is an interval too}\,.
$$
\end{cor}
\duk
Let $I$ and $f$ be as stated. Let $J\sus I$ be a~subinterval, $f(a)\ne f(b)$ 
be in $f[J]$ and let $c$ lie between $f(a)$ and $f(b)$. We may assume that 
$a<b$ because the case $a>b$ is treated similarly. By 
Theorem~\ref{thm_deriDarboux} there is a~$d\in(a,b)$ such that $f(d)=c$. Since 
$a<b$ are in the interval $J$, also $d\in J$. Thus $c=f(d)\in f[J]$ and $f[J]$ is an interval. 
\kduk

\begin{exer}\label{ex_troskuLogiky}
Give an example of a~function $f\in\mathcal{F}(M)$ such that $M$ and 
$f[M]$ are intervals, but there is an interval $I\sus M$ such that $f[I]$ is 
not an interval.    
\end{exer}

\begin{exer}\label{ex_areEqi}
Theorem~\ref{thm_deriDarboux} and Corollary~\ref{cor_Darb} are equivalent (one can be easily deduced from the other).   
\end{exer}

The following corollary of Corollary~\ref{cor_Darb} is immediate.

\begin{cor}[empty $\int(f)$]\label{cor_Darbouxe}
If $I$ is a~nontrivial interval and $f\in\mathcal{F}(I)$ is such that for 
some subinterval $J\sus I$ the image $f[J]$ is not an interval, 
\underline{then} 
$${\textstyle
\int(f)=\emptyset\,.
}
$$
\end{cor}

\noindent
{\em $\bullet$ Continuity of a~function and its primitive. }This point 
sometimes leads to confusion. Recall that if $F,f\in\mathcal{R}$ are 
functions such that $F=\int f$, then $F$
is continuous (by Proposition~\ref{prop_vlDerimplSpoj}) 
but $f$ need not be. Indeed, in the proof of Theorem~\ref{thm_nespDer} we 
constructed a~set $N\sus\R$ and a~function $F\in\mathcal{F}(N)$ (called $f$ there) such that 
$$
\text{$0\in N\ne\{0\}$, 
$F'(0)=0$ and $F'(x)=1$ for every 
$x\in N\setminus\{0\}$}\,.
$$
Thus the function $f\in\mathcal{F}(N)$ defined by $f(0)=0$ and $f(x)=1$ for 
every $x\in N\setminus\{0\}$ is discontinuous (Exercise~\ref{ex_whyDisc}) and 
$F=\int f$.

\begin{exer}\label{ex_whyDisc}
Why is $f$ discontinuous?    
\end{exer}
Another and better known example is in Exercise~\ref{ex_znovuTenPr}.

\medskip\noindent
{\em $\bullet$ Global primitive and multiplication. }We extend the well known formula for integration by parts from intervals to general domains. For two sets $A,B\sus\mathcal{R}$ we set, like for addition, 
$$
A-B\equiv\{f-g\cc\;f\in A,\,g\in B\}\,.
$$
If $A=\emptyset$ or $B=\emptyset$, then $A-B=\emptyset$.

\begin{thm}[integration by parts]\label{thm_inteBart}
Let $f,g,F,G\in\mathcal{R}$ be functions 
such that $F=\int f$ and $G=\int g$. \underline{Then}
$$
{\textstyle
\int(fG)\supset\{FG\}-\int(Fg)\,.
}
$$
\end{thm}
\duk
If $\int(Fg)=\emptyset$ or $\{\emptyset_f\}$, the inclusion trivially 
holds. We take any function $H\in\int(Fg)$ with $H\ne\emptyset_f$. 
We have
$$
M\equiv M(Fg)=M(FG)=M(fG)=M(f)\cap M(g)
$$
and $M\sus L(M)$. For every $a\in M$ we have, by part~1 of Theorem~\ref{thm_LeibnizFmle} and  Exercise~\ref{ex_sameForMinus}, that
\begin{eqnarray*}
(FG-H)'(a)&=&F'(a)G(a)+F(a)G'(a)-H(a)\\
&=&f(a)G(a)+F(a)g(a)-F(a)g(a)\\
&=&f(a)G(a)\,.
\end{eqnarray*}
Thus $FG-H\in\int(fG)$. 
\kduk
\vspace{-3mm}
\begin{exer}\label{ex_samNajdi}
Give an example of functions $f$, $g$, $F$ and $G$ for which the inclusion is 
strict.    
\end{exer}

We describe a~situation when the integration by parts formula holds 
exactly.


\begin{prop}[exact integration by parts]\label{prop_exaPerPer}
Let $f,g,F,G$ in $\mathcal{R}$ be functions such that $F=\int f$, $G=\int g$, $\int(Fg)\ne\emptyset$ and both domains $M(f)$ and $M(g)$ are intervals. \underline{Then} we have the equality of sets
$$
{\textstyle
\int(fG)=\{FG\}-\int(Fg)\,.
}
$$
\end{prop}
\duk
We take a~function $H\in\int(Fg)$ and since 
$$
M\equiv M(fG)=M(FG)=M(Fg)=M(f)\cap M(g)
$$
is an interval, 
\kduk



\section[Primitives of uniformly continuous functions]{${}^*$Primitives of UC functions}\label{sec_twoKRint}

In this section we prove Theorem~\ref{thm_primUC}. Our main tool is an extension of the Riemann integral. 

\medskip\noindent
{\em $\bullet$ tagged partitions of bounded sets. }Suppose that $M\sus\R$ is 
a~bounded set with at least two elements. By a~\underline{tagged partition\index{tagged partition of a~set|emph}} of $M$ we mean a~pair
$$
T=(\overline{p},\,\overline{t})\,\text{ where }\, \overline{p}=\langle a_0<a_1<\ds<a_n\rangle\,\text{ and }\,\overline{t}=\langle t_1,\,\ds,\,t_n\rangle
$$
are such that $n\in\N$, $a_0=\inf(M)$, $a_n=\sup(M)$, $t_i\in[a_{i-1},a_i]\cap 
M$ if this intersection is nonempty, and 
$t_i=\emptyset$ if it is empty. 
We refer to the intervals $[a_{i-1}]$ as to \underline{subintervals\index{tagged partition of a~set!subintervals|emph}} of $T$.
For $f\in\mathcal{F}(M)$ we define the \underline{extended Riemann sum\index{extended Riemann sum|emph}} 
corresponding to $T$ and $f$ by
$${\textstyle
R^*(T,\,f)\equiv\sum_{i=1}^n(a_i-a_{i-1})\cdot f(t_i)\,\text{ where }\,f(\emptyset)\equiv0\,.
}
$$
Thus subintervals disjoint to $M$ contribute nothing to the sum.

\begin{exer}\label{ex_nejakaUlo}
    
\end{exer}

\noindent
{\em $\bullet$ Stuffings of sets. }We prove by means of them the 
existence of the extended Riemann integral.

\begin{defi}[stuffing]\label{def_stuff}
Let $M\sus\R$ be bounded and have at least two elements, $a\equiv\inf(M)$ and
$b\equiv\sup(M)$, so that $a<b$. A~\underline{stuffing\index{stuffing|emph}} of the set $M$ is an at most countable system
$$
\{J_i\cc\;i\in S\}
$$
of nonempty open intervals $J_i$ that are pairwise disjoint and have the following 
properties.
\begin{enumerate}
\item We have $\bigcup_{i\in S}J_i\sus[a,b]\setminus M$.
\item If $c<d$ and $(c,d)\sus[a,b]\setminus\bigcup_{i\in S}J_i$ then $M$ is dense in $(c,d)$.
\end{enumerate}
\end{defi}

\begin{prop}[stuffings exist]\label{prop_stuffEx}
Any bounded and at least two-element real set has a~stuffing.     
\end{prop}
\duk
Let $M$, $a$ and $b$ be as in Definition~\ref{def_stuff}. We define 
a~stuffing of $M$ by going through the
elements of the countable set $[a,b]_{\Q}$ one by one. We initialize 
the index set by $S_0\equiv\emptyset$ and order $[a,b]_{\Q}$ in a~sequence
$$
(\al_1,\,\al_2,\,\ds)\,.
$$
In step $n\in\N$ we assume that the nonempty open and disjoint intervals 
$J_i$, $i\in S_{n-1}$, with property~1 are already 
defined. If $\al_n\in\bigcup_{i\in S_{n-1}}J_i$, we set $S_n\equiv S_{n-1}$, 
keep the intervals and proceed to step $n+1$. If $\al_n\not\in\bigcup_{i\in S_{n-1}}J_i$ but there is no open interval $I$ such that
$${\textstyle
\al_n\in I\sus[a,\,b]\setminus \big(M\cup\bigcup_{i\in S_{n-1}}J_i\big)\,,
}
$$
we do the same. If $\al_n\not\in\bigcup_{i\in S_{n-1}}J_i$ 
and there is an interval $I$ as stated, we take $I$ to be inclusion-wise largest (Exercise~\ref{ex_whyItEx}),
set $S_n\equiv S_{n-1}\cup\{n\}$, keep the intervals, add to them the 
interval $J_n\equiv I$ and proceed to step $n+1$.

After $\omega$ steps we define $S\equiv\bigcup_{n\in\N}S_n$. It is 
clear that the system
$$
\{J_i\cc\;i\in S\}
$$
consists of nonempty open intervals that are disjoint and have property~1. To 
prove that it has also property~2, we assume for contradiction that $c<c'<d'<d$
are such real numbers that 
$${\textstyle
(c,d)\sus[a,b]\setminus\bigcup_{i\in S}J_i
}
$$
but $M\cap(c',d')=\emptyset$. We take the minimum $n\in\N$ such that
$\al_n\in(c',d')$. We see that in step $n$ we had
$$
{\textstyle
\al_n\in (c',\,d')\sus[a,\,b]\setminus \big(M\cup\bigcup_{i\in S_{n-1}}J_i\big)
}
$$
but we did not add to the current intervals any open interval contaaining $\al_n$, in contradiction with the procedure.
\kduk
\vspace{-3mm}
\begin{exer}\label{ex_whyItEx}
Why does such inclusion-wise largest interval $I$ exist?    
\end{exer}













==> lec11.tex <==
\chapter[Newton integral. Primitives of rational 
functions]{Newton integral. Primitives of rational 
functions}\label{chap_pr11}

















==> lec12.tex <==
\chapter[Riemann integral. Transcendence of the number $\mathrm{e}$]{Riemann integral. Transcendence of $\mathrm{e}$}\label{chap_pr12}

















==> lec13.tex <==
\chapter[Riemann integral. Henstock--Kurzweil integral]{Riemann integral. 
Henstock--Kurzweil integral}\label{chap_pr13}

















==> lec14.tex <==
\chapter[More applications of Riemann integral]{More applications of Riemann integral}\label{chap_pr14}

The last chapter of this treatise is based on the lecture
\begin{quote}
\url{https://kam.mff.cuni.cz/~klazar/MAI24_pred14.pdf}    
\end{quote}
I gave on May 23, 2024. Section~\ref{sec_14_1} is devoted to
lengths of curves and to their computation via Riemann integrals. In
the extending Section~\ref{sec_14_2} we treat areas of sets in the plane
$\R^2$.

\section[Length of curves]{Length of curves}\label{sec_14_1}

In this section we obtain formulas in terms of Riemann integrals 
$\int_a^b f$ for lengths of (tame) curves in $\R^d$. We begin by 
defining these notions. 

\medskip\noindent
{\em $\bullet$ Curves in $d$ dimensions. }Let $d\in\N$. Curves in the 
$d$-dimensional Euclidean space $\R^d$ are simply maps from intervals $[a,b]$ to $\R^d$. The adjective ``Euclidean'' reminds us that $\R^d$ is endowed with the distance function
$${\textstyle
\|\overline{x}-\overline{y}\|=
\sqrt{\sum_{j=1}^d(x_j-y_j)^2}\,.
}
$$
Here $\overline{x}=(x_1,x_2,\ds,x_d)$
and $\overline{y}=(y_1,y_2,\ds,y_d)$ are two points in $\R^d$. 

\begin{defi}[curves]\label{def_curves}
Let $d\in\N$. 
A~\underline{curve\index{curve@curve in $\R^d$|emph}} in $\R^d$ is any 
function (congruent to a~function)
$$
\varphi\cc I\equiv[a,\,b]\to\R^d\,,
$$
where $a<b$ are real numbers.
\end{defi}
Sometimes one means by a~curve its image $\varphi[I]$ ($\sus\R^d$) 
but we distinguish between curves and their images. An example
of a~curve in $\R^1$ is the identity map $\varphi(x)=x\cc[a,b]\to\R$. 

\begin{exer}\label{ex_uppHalfC}
Write in terms of sine and cosine a~formula for a~curve $g(t)$ in $\R^2$ with
an image equal to the graph $G_f$ of the function $f(x)\equiv\sqrt{1-x^2}$. Write
another formula for such a~curve $h(x)$ in terms of $f(x)$.
\end{exer}

\begin{exer}\label{ex_segment}
Write a~formula for a~curve $f(t)$ in $\R^d$  with an image equal to the
straight segment that joins the points $\overline{a}\equiv(0,0,\ds,0)$ 
and $\overline{b}\equiv(1,1,\ds,1)$.
\end{exer}

\begin{exer}\label{ex_helix}
Write a~formula for a~curve $\varphi(t)$ in $\R^3$  with an image equal to the helix that
winds in five revolutions around the segment $(0,0,0)(1,0,0)$ in distance
$2$.
\end{exer}

\noindent
{\em $\bullet$ The length of a~curve. }This length always exists and is an element of the set $[0,+\infty]\equiv[0,+\infty)\cup
\{+\infty\}$.

\begin{defi}[lengths of curves]\label{def_lenCur}
Let $\varphi\cc[a,b]\to\R^d$ be a~curve in $\R^d$. We define the \underline{length\index{length of a~curve|emph}\index{curve@curve 
in $\R^d$!length of|emph}} of $\varphi$ as the supremum
$${\textstyle
\ell(\varphi)\equiv
\sup\big(
\big\{
\sum_{j=1}^n\|\varphi(t_i)-\varphi(t_{i-1})\|\cc\;
a=t_0<t_1<\ds<t_n=b
\big\}
\big)\,,
}
$$
taken in the linear order $(\R^*,<)$.
\end{defi}
The length $\ell(\varphi)$ of $\varphi$ may be $+\infty$ and is the
supremum of lengths of all broken lines that join the points
$\varphi(a)$ and $\varphi(b)$ and are inscribed in the image of $\varphi$. 

\begin{exer}\label{ex_zeroLe}
Find all curves in $\R^d$ with length zero.    
\end{exer}

\begin{exer}\label{ex_LeIdCu}
Determine the lengths of the identity curves in $\R^1$ mentioned after
Definition~\ref{def_curves}.    
\end{exer}

\noindent
{\em $\bullet$ Properties of $\ell(\varphi)$. }We obtain lower and upper bounds for $\ell(\varphi)$, and some transformations of $\R^d$ preserving $\ell(\varphi)$. 

Let 
$$
\varphi=(\varphi_1,\,\varphi_2,\,\ds,\,\varphi_d)\cc[a,b]\to\R^d
$$ 
be a~curve. We say that $\varphi$ is \underline{unbounded\index{curve@curve in $\R^d$!unbounded|emph}} if the 
set 
$$
\{\|\varphi(x)-\varphi(y)\|\cc\;x,\,y\in[a,b]\}\ \  (\sus[0,+\infty)) 
$$
is unbounded. We say that $\varphi$ is \underline{monotone\index{curve@curve in $\R^d$!monotone|emph}} if each of the $d$ functions $\varphi_i$ ($\in\mathcal{F}([a,b])$) is monotone.

\begin{prop}[bounds on length]\label{prop_boundLeng}
Let $\varphi\cc[a,b]\to\R^d$ be a~curve in $\R^d$, and let $\overline{a}\equiv\varphi(a)$ and $\overline{b}\equiv\varphi(b)$. The following holds.
\begin{enumerate}
\item Always $\ell(\varphi)\ge\|\overline{b}-\overline{a}\|$. 
\item If the curve $\varphi$ is unbounded \underline{then} $\ell(\varphi)=+\infty$.
\item If the curve $\varphi$ is monotone \underline{then}
$$
{\textstyle
\ell(\varphi)\le\sum_{j=1}^d|b_j-a_j|\,.
}
$$
\end{enumerate}    
\end{prop}
\duk
Let $\varphi$, $\overline{a}$ and $\overline{b}$ be as stated.

1. Let $a=t_0<t_1<\ds<t_n=b$ be any partition of $[a,b]$ and let 
$\overline{a}_i\equiv\varphi(t_i)$. By
the triangle inequality in $\R^d$ (Exercise~\ref{ex_trInRd}) we have
$$
{\textstyle
\|\overline{b}-\overline{a}\|=
\big\|\sum_{i=1}^n(\overline{a}_i-
\overline{a}_{i-1})\big\|\le
\sum_{i=1}^n\|\overline{a}_i-
\overline{a}_{i-1}\|.
}
$$
Using Definition~\ref{def_lenCur} we get the lower bound.

2. 
\kduk
\vspace{-3mm}
\begin{exer}\label{ex_shortest}
If in part~1 of Proposition~\ref{prop_boundLeng} the 
equality holds, then the image of $\varphi$ is a~subset of the segment 
$\overline{a}\overline{b}$.    
\end{exer}

\begin{exer}\label{ex_trInRd}
Prove the triangle inequality in $\R^d$: $\|\overline{a}+\overline{b}\|
\le\|\overline{a}\|+\|\overline{b}\|$.    
\end{exer}

Let 
$$
\varphi=(\varphi_1,\,\varphi_2,\,\ds,\,\varphi_d)\cc[a,b]\to\R^d
$$ 
be a~curve and $\overline{a}\in\R^d$. By $\varphi+\overline{a}$ we mean the curve $\psi\cc[a,b]\to\R^d$ such that
$\psi_i(t)=\varphi_i(t)+a_i$ for every $i\in[d]$. Similarly, if 
$M=(m_{i,j})\in\R^{d\times d}$ is a~$d\times d$ real matrix, then by 
$\varphi\cdot M$ we mean the curve $\psi\cc[a,b]\to\R^d$ such that for every $j\in[d]$, 
$$
{\textstyle
\psi_j(t)=\sum_{i=1}^d\varphi_i(t)\cdot m_{i,\,j}\,.
}
$$
Recall that the matrix $M$ is \underline{orthonormal\index{orthonormal matrix|emph}} if $M^TM=I$, 
the transpose of $M$ is inverse to $M$. Orthonormal matrices determine 
rotations in $\R^d$ around the origin. If $\psi\cc[c,e]\to\R^d$ is 
another curve in $\R^d$, we say that 
$\psi$ \underline{prolongs\index{curve@curve 
in $\R^d$!prolongs another curve|emph}} $\varphi$ if $b=c$ and 
$\varphi(b)=\psi(c)$. We then write $\varphi\psi$ for the curve 
$\theta\cc[a,e]\to\R^d$ given by $\theta(t)=\varphi(t)$ for 
$t\in[a,b]$, and by $\theta(t)=\psi(t)$ for $t\in[c,e]$.


\begin{prop}[preservation of length]\label{prop_preserLeng}
Suppose that $\varphi\cc[a,b]\to\R^d$ 
and $\psi\cc[c,e]\to\R^d$
are two curves in $\R^d$ such that $\psi$ prolongs $\varphi$. The following holds.
\begin{enumerate}
\item For every vector $\overline{a}\in\R^d$ we have $\ell(\varphi+\overline{a})=\ell(\varphi)$.
\item For every orthonormal matrix $M\in\R^{d\times d}$ we have $\ell(\varphi\cdot M)=\ell(\varphi)$.
\item It is true that $\ell(\varphi\psi)=\ell(\varphi)+\ell(
\psi)$.
\end{enumerate}
\end{prop}
\duk

\kduk

\noindent
{\em $\bullet$ An infinitely long continuous curve. }

\medskip\noindent
{\em $\bullet$ The first formula for the length $\ell(\varphi)$. }

\begin{thm}[1st formula for $\ell(\varphi)$]\label{thm_1stForLen}
Let $d\in\N$ and 
$$
\varphi=(\varphi_1,\,\varphi_2,\,\ds,\,\varphi_d)\cc[a,b]\to\R^d
$$
be a~curve in $\R^d$ such that $\varphi_i'\in\mathcal{R}([a,b])$ for 
every $i\in[d]$. \underline{Then}
$$
\ell(\varphi)=\int_a^b{\textstyle
\sqrt{\sum_{i=1}^d(\varphi_i')^2}\,.
}
$$
\end{thm}
\duk

\kduk

\noindent
{\em $\bullet$ The second formula for the length $\ell(\varphi)$. }


\section[Area of plane sets]{${}^*$Area of plane sets}\label{sec_14_2}

The purpose of this section is to give sense to the standard 
``theorem'' in courses of elementary analysis which says that the area under the graph of a~nonnegative function 
$f\in\mathcal{R}([a,b])$ is
$\int_a^b f$. We begin, paradoxically,  by showing that there exist sets in the plane to which no area can be assigned.  

\medskip\noindent
{\em $\bullet$ Plane sets with no area. }Length of curves, introduced 
in the previous section, is defined for every curve. In contrast, it is 
well known that the area function with minimal desirable
properties cannot be defined for all subsets of $\R^2$. We prove it
now. 

Let $[0,+\infty]\equiv[0,+\infty)\cup
\{+\infty\}$ and 
$A\cc\mathcal{P}(\R^2)\to[0,+\infty]$ be a~function defined on all plane 
sets, whose values are nonnegative real numbers or $+\infty$.
We say that $A$ is \underline{horizontally 
shift-invariant\index{horizontally shift-invariant function, HSI|emph}}, 
or HSI, if for every set $X\sus\R^2$ and number $s\in\R$,
$$
A(X+s)=A(X)\,,
$$
where $X+s\equiv\{(x+s,y)\cc\;(x,y)\in X\}$. We say that $A$ is 
\underline{$\sigma$-additive\index{sigma additive@$\sigma$-additive function|emph}}

\begin{defi}[areas of bounded sets]
Let $X\sus B$ where $X$ is a~set and $B\sus\R^2$ is a~box. We define 
the \underline{$B$-area\index{area!barea@$B$-area|emph}} of $X$ as the integral over $B$
$${\textstyle
\mathrm{area}_B(X)\equiv
\int_B\chi_{B,\,X}
}
$$
of the $B$-characteristic 
function $\chi_{B,X}\cc B\to\{0,1\}$  of $X$, if this integral exists.
\end{defi}

\begin{prop}[independence on $B$]
If $X\sus B\cap B'$  where $X$ is a~set and $B,B'\sus\R^2$ are boxes, \underline{then}
$$
\mathrm{area}_B(X)=
\mathrm{area}_{B'}(X)
$$
whenever either areas exists.
\end{prop}

\begin{defi}[areas of general sets]\label{def_areaGenSet}
Let $X\sus\R^2$ be a~set and $P=\{P_1,P_2,\ds\}$ be a~partition of $X$ in countably many bounded sets. We define
the \underline{$P$-area\index{area!parea@$P$-area|emph}} of $X$ as the sum
$${\textstyle
\mathrm{area}^P(X)\equiv
\sum\mathrm{area}(P_n)\ \ (\in[0,\,+\infty)\cup\{+\infty\})\,.
}
$$
\end{defi}

\section[Newton's shell theorems in the plane]{${}^*$Newton's shell theorems in the plane}

\section[Volume of solids]{Volume of solids}













